Closed-form modeling of neuronal spike train statistics using multivariate Hawkes cumulants

We derive exact analytical expressions for the cumulants of any orders of neuronal membrane potentials driven by spike trains in a multivariate Hawkes process model with excitation and inhibition. Such expressions can be used for the prediction and sensitivity analysis of the statistical behavior of the model over time, and to estimate the probability densities of neuronal membrane potentials using Gram-Charlier expansions. Our results are shown to provide a better alternative to Monte Carlo estimates via stochastic simulations, and computer codes based on combinatorial recursions are included.

==> tkz-arith.tex <==
\def\fileversion{0.999 c}
\def\filedate{2010/08/21}
%  Author Alain Matthes
%<--------------------------------------------------------------------------–>
%% Objet :  tools for arithmetic 

%<--------------------------------------------------------------------------–>
%    [2010/04/16 v0.99c integers numbers]
%<--------------------------------------------------------------------------–>
\newcount\tkz@prim@a
\newcount\tkz@prim@b
\newcount\tkzprim@a
\newcount\tkzprim@b
\newcount\tkzprim@r
\newcount\tkzprim@q
\newcount\tkzprim@n
\newcount\tkzprim@d
\newcount\tkzprim@last
\newcount\NbOfPrimFactor

\newif\iftkz@prime
\newif\iftkz@unknown
\newif\iftkz@test@
\newif\iftkzIsAPrim 
\newif\iftkzIsAFactor

\NbOfPrimFactor0 %

% tkz@loop (from plain.tex and pgf)

\def\tkz@loop#1\tkz@repeat{\def\tkz@body{#1}\tkz@iterate}
\def\tkz@iterate{\tkz@body \let\tkz@next\tkz@iterate \else\let\tkz@next\relax\fi \tkz@next}
\let\tkz@repeat=\fi % this makes \loop...\if...\repeat skippable      
%<--------------------------------------------------------------------------–>
%                            arithmetic tools 
%<--------------------------------------------------------------------------–>
%                          Mod
% ne sera plus nécessaire avec pgf 2 cvs
\ifdefined\pgfmathdeclarefunction
\else
\def\pgfmath@parsefunction@Mod{%
  \expandafter\pgfmath@parsefunction@Mod@}
\def\pgfmath@parsefunction@Mod@(#1,{%
  \pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
  \let\pgfmath@parsepostgroup\pgfmath@parsefunction@Mod@@
  \pgfmath@startparsegroup}
\def\pgfmath@parsefunction@Mod@@{%
  \edef\pgfmath@secondoperand{\pgfmathresult}%
  \pgfmathMod@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
  \pgfmath@postfunction}
% \pgfmathmod
% Calculate #1 Mod #2.
\def\pgfmathMod#1#2{%
  \edef\pgfmath@marshal{%
    \noexpand\pgfmathparse{#2}
    \noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
    \noexpand\pgfmathparse{#1}%
  }%
  \pgfmath@marshal%
  \pgfmathMod@{\pgfmathresult}{\pgfmath@arg}%
}
\def\pgfmathMod@#1#2{%
  \begingroup
    \pgfmath@xa#1pt%
    \pgfmath@xb#2pt%
    \pgfmath@x\pgfmath@xa%
    \c@pgfmath@counta\pgfmath@xa%
    \c@pgfmath@countb\pgfmath@xb%
    \divide\c@pgfmath@counta\c@pgfmath@countb%
    \multiply\pgfmath@xb\c@pgfmath@counta%
    \advance\pgfmath@x-\pgfmath@xb%
        \pgfmath@xb#2pt%
        \ifdim\pgfmath@x<0pt\relax%
       \advance\pgfmath@x\pgfmath@xb\relax%
     \fi
    \pgfmath@returnone\pgfmath@x%
  \endgroup
}
\fi
%<--------------------------------------------------------------------------–>
%                    find factors of an integer
%<--------------------------------------------------------------------------–>

\newcommand*{\tkz@factors}[1]{%
\tkzprim@b#1 
\tkzprim@d2\relax
%<--------------------------------------------------------------------------–>
\tkz@test@true 
\@whilesw\iftkz@test@ \fi{%
\ifodd\tkzprim@b  \tkz@test@false 
\else
 \divide\tkzprim@b by2 %
  $\number\tkzprim@d\ $ 
\fi}%
\tkzprim@last=1 %
  \loop  \ifnum\tkzprim@b>1  
    \tkzprim@d\tkzprim@last\relax
    \tkzprim@r1\relax
%<--------------------------------------------------------------------------–>
\tkz@loop\ifnum\tkzprim@r>0 % 
            \tkzprim@last\tkzprim@d
            \advance\tkzprim@d by2\relax% on commence par 3
            \tkzprim@a\tkzprim@b% macro mod !!
            \tkzprim@r\tkzprim@a%
            \divide\tkzprim@a by \tkzprim@d
            \multiply\tkzprim@a by\tkzprim@d %
            \advance\tkzprim@r by-\tkzprim@a%
     \tkz@repeat % fin du whiledo on a le reste
    \divide\tkzprim@b by\tkzprim@d\relax
    $\number\tkzprim@d\ $%  affiche le facteur
\repeat% fin du premier whiledo
}%    
%<--------------------------------------------------------------------------–>
%                  search factors   % if prime number tkzIsAPrimtrue        
%<--------------------------------------------------------------------------–>
\def\tkzfactors#1{%
\tkzprim@b#1 
\tkzIsAPrimfalse
\tkz@primality{\tkzprim@b}% 
\iftkzIsAPrim
   \number\tkzprim@b\ % prime number
\else we can found factors
\tkz@factors{#1} 
\fi
}%
%<--------------------------------------------------------------------------–>
% \iftkzIsAPrim to test
%<--------------------------------------------------------------------------–>
\def\tkz@primality#1{%
\tkz@unknowntrue
\tkzprim@n =#1
\ifnum\tkzprim@n =1 \tkz@primefalse\tkz@unknownfalse\fi
\ifnum\tkzprim@n =2 \tkz@primetrue\tkz@unknownfalse\fi
\ifnum\tkzprim@n =3 \tkz@primetrue\tkz@unknownfalse\fi
\iftkz@unknown
\tkzprim@d=2 
\tkzprim@a=\tkzprim@n  %
     \divide\tkzprim@a by\tkzprim@d %
     \multiply\tkzprim@a by\tkzprim@d %
\ifnum\tkzprim@a=\tkzprim@n  \global\tkz@primefalse\tkz@unknownfalse\fi
 \fi
\iftkz@unknown
\tkzprim@d=3 \global\tkz@primetrue
 \tkz@loop
 \tkzprim@a=\tkzprim@n  \divide\tkzprim@a by\tkzprim@d
  \ifnum\tkzprim@a>\tkzprim@d \tkz@unknowntrue\else\tkz@unknownfalse\fi
    \multiply\tkzprim@a by\tkzprim@d
  \ifnum\tkzprim@a=\tkzprim@n  \global\tkz@primefalse\tkz@unknownfalse\fi
  \iftkz@unknown\advance\tkzprim@d by 2 %
 \tkz@repeat
\fi
\iftkz@prime\tkzIsAPrimtrue\else\tkzIsAPrimfalse\fi
}%
%<--------------------------------------------------------------------------–>
% #2 divide #1 ?
%<--------------------------------------------------------------------------–>
\def\tkzFindFactor#1#2{% 
\tkzprim@a#1 \tkzprim@b#2
\tkzprim@r#1    
\divide\tkzprim@a by\tkzprim@b%
\multiply\tkzprim@a by\tkzprim@b% 
\advance\tkzprim@r by-\tkzprim@a%
\ifnum\tkzprim@r=0 \tkzIsAFactortrue\else\tkzIsAFactorfalse\fi}% 
%<--------------------------------------------------------------------------–>
% find pgcd of #1 and #2 result in \tkz@mathresult and \theprim@a
%<--------------------------------------------------------------------------–>
\def\tkz@pgcd#1#2{%   test si l'un est nul

\tkzprim@a#1 \tkzprim@b#2
\tkz@test@true
\ifnum\tkzprim@a=0 \tkz@test@false\tkzprim@a\tkzprim@b\fi
\ifnum\tkzprim@b=0 \tkz@test@false\tkzprim@b\tkzprim@a\fi  
\@whilesw\iftkz@test@ \fi{%
\ifnum\tkzprim@a=\tkzprim@b\tkz@test@false
\else
 \ifnum\tkzprim@a>\tkzprim@b%
 \advance \tkzprim@a by-\tkzprim@b
\else \advance \tkzprim@b by-\tkzprim@a\fi
\fi}%
\edef\tkz@mathresult{\number\tkzprim@a}}%
%<--------------------------------------------------------------------------–>
%                   Simplification d'une fraction
% #2 if #2<>1 then frac with pi
%<--------------------------------------------------------------------------–>
\def\tkz@reducfrac#1#2{%
\ifnum#1<0\relax%
   \tkz@prim@a 0 
   \advance\tkz@prim@a by -#1
 \else
    \tkz@prim@a#1 %
 \fi
  \tkz@prim@b#2 %
  \tkz@pgcd{\tkz@prim@a}{\tkz@prim@b}% 
 \ifnum\tkz@prim@a=0%
   \tkz@prim@a#1 %
   \tkz@prim@b#2 %
 \else 
   \tkz@prim@a#1 
   \tkz@prim@b#2 
   \divide \tkz@prim@a by\tkz@mathresult   
   \divide \tkz@prim@b by\tkz@mathresult  
\fi
\def\tkz@rfrac{$\frac{\the\tkz@prim@a\pi}{\the\tkz@prim@b}$}
% modif for pi
 \ifnum\tkz@prim@a=0%
    \global\def\tkz@rfrac{}%
 \else
 \ifnum\tkz@prim@b=1 %
    \ifnum\tkz@prim@a=1 %
      \global\def\tkz@rfrac{$\scriptstyle{\pi}$}%
      \else
       \ifnum\tkz@prim@a=-1%
          \global\def\tkz@rfrac{$\scriptstyle{-\pi}$}%
        \else
          \global\def\tkz@rfrac{$\scriptstyle{\the\tkz@prim@a\pi}$}%
       \fi\fi
 \else 
   \ifnum\tkz@prim@a=1 %
       \global\def\tkz@rfrac{$\frac{\pi}{\the\tkz@prim@b}$}%
     \else
       \ifnum\tkz@prim@a=-1 %
          \global\def\tkz@rfrac{$\frac{-\pi}{\the\tkz@prim@b}$}%
        \else 
           \global\def\tkz@rfrac{$\frac{\the\tkz@prim@a\pi}{\the\tkz@prim@b}$}%
 \fi\fi\fi\fi
}%
\endinput



